Acquiescence Bias in Large Language Models

Acquiescence bias, i.e. the tendency of humans to agree with statements in surveys, independent of their actual beliefs, is well researched and documented. Since Large Language Models (LLMs) have been shown to be very influenceable by relatively small changes in input and are trained on human-generated data, it is reasonable to assume that they could show a similar tendency. We present a study investigating the presence of acquiescence bias in LLMs across different models, tasks, and languages (English, German, and Polish). Our results indicate that, contrary to humans, LLMs display a bias towards answering no, regardless of whether it indicates agreement or disagreement.

==> fig.tex <==
\begin{figure*}

\foreach \condition in {yesno_prompt,agree_prompt,negated_agree_prompt,disagree_prompt}{
\foreach \model in {Llama-3.1-8B,Mistral-Small-24B,Llama-3.3-70B,gpt-4o-2024-08-06}
    {\begin{subfigure}{0.25\textwidth}
    \centering
        \begin{tikzpicture}
        \begin{axis}[
                width = \textwidth,
                height=6cm,
                tick style={draw=none},
                tick align=inside,axis x line* = middle,
                y axis line style={draw=none},
                ybar,
                ymin=-95,
                ymax = 95,
                %ymax=\ifthenelse{\equal{\condition}{disagree_prompt}}{600}{95},
                ymajorgrids=true,
                major grid style={line width=.2pt,draw=gray!50},
                bar width=4pt,
                ylabel=\ifthenelse{\equal{\model}{Llama-3.1-8B}}{\expUScore{\condition}}{~},
                yticklabel=\ifthenelse{\equal{\model}{Llama-3.1-8B}}{$\pgfmathprintnumber{\tick}$\%}{\empty},
                symbolic x  coords={definition_classification, cuad_cap_on_liability, cuad_no-solicit_of_customers,  contract_nli_explicit_identification, hearsay, contract_nli_confidentiality_of_agreement, cuad_non-compete, agb-de, clauses-pl, overall},
                xticklabels = data,
                title=\ifthenelse{\equal{\condition}{yesno_prompt}}{\expUScore{\model}}{~},
                enlarge x limits=3.0,
                cycle list name=Set3
            ]
            \pgfplotsinvokeforeach {definition_classification, cuad_cap_on_liability, cuad_no-solicit_of_customers,  contract_nli_explicit_identification, hearsay, contract_nli_confidentiality_of_agreement, cuad_non-compete, agb-de,clauses-pl,overall} {
            \addplot+ [ybar, fill,
               discard if not={condition}{\condition},
               discard if not={model}{\model},
               discard if not={task}{####1}
               ] table [col sep=comma, y=positive_change, x=task] {evaluation.csv};
               \label{####1}
           }
        \end{axis}
        \end{tikzpicture}
    \end{subfigure}}
}

\caption{Change in the number of instances that have been classified as positive for each model and prompting strategy by task (definition\_classification \ref{definition_classification}, cuad\_cap\_on\_liability \ref{cuad_cap_on_liability}, cuad\_no-solicit\_of\_customers \ref{cuad_no-solicit_of_customers}, contract\_nli\_explicit\_identification \ref{contract_nli_explicit_identification}, hearsay \ref{hearsay}, contract\_nli\_confidentiality\_of\_agreement \ref{contract_nli_confidentiality_of_agreement}, cuad\_non-compete \ref{cuad_non-compete}, agb-de \ref{agb-de}, clauses-pl \ref{clauses-pl}, overall \ref{overall}
) \label{fig:pos}}

\end{figure*}
